Scale Efficiently: Insights from Pre-training and Fine-tuning Transformers

There remain many open questions pertaining to the scaling behaviour of Transformer architectures. These scaling decisions and findings can be critical, as training runs often come with an associated computational cost which have both financial and/or environmental impact. The goal of this paper is to present scaling insights from pretraining and finetuning Transformers. While Kaplan et al. presents a comprehensive study of the scaling behaviour of Transformer language models, the scope is only on the upstream (pretraining) loss. Therefore, it is still unclear if these set of findings transfer to downstream task within the context of the pretrain-finetune paradigm. The key findings of this paper are as follows: (1) we show that aside from only the model size, model shape matters for downstream fine-tuning, (2) scaling protocols operate differently at different compute regions, (3) widely adopted T5-base and T5-large sizes are Pareto-inefficient. To this end, we present improved scaling protocols whereby our redesigned models achieve similar downstream fine-tuning quality while having 50\% fewer parameters and training 40\% faster compared to the widely adopted T5-base model. We publicly release over 100 pretrained checkpoints of different T5 configurations to facilitate future research and analysis.

==> old.tex <==
% \citet{kaplan2020scaling} argues that the performance of a Transformer neural language model strongly depends on the model \emph{size}, but only weakly on the model \emph{shape}.
% Our work empirically confirms their results for upstream training, but then reveals a striking discrepancy when fine-tuning: downstream task performance is strongly influenced by model shape (e.g. depth and width).
% We find that widely adopted models including \emph{T5-Base}, \emph{T5-Large} and \emph{T5-XL/XXL}~\citep{raffel2019exploring} are inefficient on a compute-performance Pareto curve. To this end, we present improved scaling protocols whereby our redesigned models achieve similar downstream fine-tuning quality while having 50\% fewer parameters and training 40\% faster.
% We conclude by demonstrating that our improved scaling protocol also holds in the vision domain and improves the Pareto efficiency of ViT~\citep{dosovitskiy2020image}.

% % Previous abstract (May 18, 2021)def3e4
% The goal of this paper is to empirically investigate scaling strategies for transformer models that are Pareto-optimal with respect to the compute-performance trade-off. Contrary to previous findings, e.g., Kaplan et al. that only considers pre-training (upstream) performance, we find that downstream performance is in fact strongly influenced by model shape (e.g., depth, width) and not only by model size. Moreover, we find that upstream perplexity might also be misleading indicator of performance of downstream transfer and therefore model building guided solely by upstream perplexity is misguided. To this end, we also find that the standard configurations for \textit{`base`} or \textit{`large`} transformers to be relatively pareto-inefficient and hence provide scaling recipes for stronger, more pareto-efficient configurations. Our study provides the first large scale analysis of Transformer model scaling behaviour with respect to both upstream and downstream performance on language understanding tasks. Moreover, we additionally show that these findings are also transferable to ViT (Vision Transformers). 
% \todo{Quantify the inefficiency of the past T5 approach.}
% \todo{Does the inefficiency come primarily from upstream (pretraining) or downstream (fine-tuning) quality?}
